Failure Transparency in Stateful Dataflow Systems (Technical Report)

Failure transparency enables users to reason about distributed systems at a higher level of abstraction, where complex failure-handling logic is hidden. This is especially true for stateful dataflow systems, which are the backbone of many cloud applications. In particular, this paper focuses on proving failure transparency in Apache Flink, a popular stateful dataflow system. Even though failure transparency is a critical aspect of Apache Flink, to date it has not been formally proven. Showing that the failure transparency mechanism is correct, however, is challenging due to the complexity of the mechanism itself. Nevertheless, this complexity can be effectively hidden behind a failure transparent programming interface. To show that Apache Flink is failure transparent, we model it in small-step operational semantics. Next, we provide a novel definition of failure transparency based on observational explainability, a concept which relates executions according to their observations. Finally, we provide a formal proof of failure transparency for the implementation model; i.e., we prove that the failure-free model correctly abstracts from the failure-related details of the implementation model. We also show liveness of the implementation model under a fair execution assumption. These results are a first step towards a verified stack for stateful dataflow systems.

==> figures/causality/invalid-intertask.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=0.75, every node/.style={scale=1},
  thick, colorGrayBase,
  timeline/.style={-{Triangle[angle=45:5]}, thick},
  message/.style={-{Triangle[angle=45:5]}, very thick, controls={+(down:0.9) and +(up:1.1)}},
  messageNode/.style={scale=0.4, circle, fill, prefix after command={\pgfextra{\tikzset{every label/.style={label distance=-1.5mm, scale=0.75}}}}},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12},
  snapshotEdge/.style={very thick, handdrawn}
]
\node[label={left:{$p_1$}},scale=0] at (0,1) {};
\draw[timeline](0,1) -- (3.5,1);
\node[label={left:{$p_2$}},scale=0] at (0,0) {};
\draw[timeline](0,0) -- (3.5,0);

\node[messageNode,label={[colorRedBase]$m_1$},colorRedBase] (m21) at (1.5,1) {};
\draw[message,colorRedBase](m21.center) to (0.5,0);
\node[messageNode,label={[colorBlueBase]$m_2$},colorBlueBase] (m22p) at (2,1) {};
\draw[message,colorBlueBase](m22p.center) to (3,0);
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/causality/invalid-intratask.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=0.75, every node/.style={scale=1},
  thick, colorGrayBase,
  timeline/.style={-{Triangle[angle=45:5]}, thick},
  message/.style={-{Triangle[angle=45:5]}, very thick, controls={+(down:0.9) and +(up:1.1)}},
  messageNode/.style={scale=0.4, circle, fill, prefix after command={\pgfextra{\tikzset{every label/.style={label distance=-1.5mm, scale=0.75}}}}},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12},
  snapshotEdge/.style={very thick, handdrawn}
]
\node[label={left:{$p_1$}},scale=0] at (0,1) {};
\draw[timeline](0,1) -- (3.5,1);
\node[label={left:{$p_2$}},scale=0] at (0,0) {};
\draw[timeline](0,0) -- (3.5,0);

\node[messageNode,label={[colorBlueBase]$m_2$},colorBlueBase] (m21) at (0.5,1) {};
\draw[message,colorBlueBase](m21.center) to (1.5,0);
\node[messageNode,label={[colorRedBase]$m_1$},colorRedBase] (m22p) at (2,1) {};
\draw[message,colorRedBase](m22p.center) to (3,0);
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/causality/original.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=0.75, every node/.style={scale=1},
  thick, colorGrayBase,
  timeline/.style={-{Triangle[angle=45:5]}, thick},
  message/.style={-{Triangle[angle=45:5]}, very thick, controls={+(down:0.9) and +(up:1.1)}},
  messageNode/.style={scale=0.4, circle, fill, prefix after command={\pgfextra{\tikzset{every label/.style={label distance=-1.5mm, scale=0.75}}}}},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12},
  snapshotEdge/.style={very thick, handdrawn}
]
\node[label={left:{$p_1$}},scale=0] at (0,1) {};
\draw[timeline](0,1) -- (3.5,1);
\node[label={left:{$p_2$}},scale=0] at (0,0) {};
\draw[timeline](0,0) -- (3.5,0);

\node[messageNode,label={[colorRedBase]$m_1$},colorRedBase] (m21) at (0.5,1) {};
\draw[message,controls={+(down:1.1) and +(up:0.9)},colorRedBase](m21.center) to (2.5,0);
\node[messageNode,label={[colorBlueBase]$m_2$},colorBlueBase] (m22p) at (1,1) {};
\draw[message,colorBlueBase](m22p.center) to (3,0);
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/causality/valid.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=0.75, every node/.style={scale=1},
  thick, colorGrayBase,
  timeline/.style={-{Triangle[angle=45:5]}, thick},
  message/.style={-{Triangle[angle=45:5]}, very thick, controls={+(down:0.9) and +(up:1.1)}},
  messageNode/.style={scale=0.4, circle, fill, prefix after command={\pgfextra{\tikzset{every label/.style={label distance=-1.5mm, scale=0.75}}}}},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12},
  snapshotEdge/.style={very thick, handdrawn}
]
\node[label={left:{$p_1$}},scale=0] at (0,1) {};
\draw[timeline](0,1) -- (3.5,1);
\node[label={left:{$p_2$}},scale=0] at (0,0) {};
\draw[timeline](0,0) -- (3.5,0);

\node[messageNode,label={[colorRedBase]$m_1$},colorRedBase] (m21) at (0.5,1) {};
\draw[message,colorRedBase](m21.center) to (1.5,0);
\node[messageNode,label={[colorBlueBase]$m_2$},colorBlueBase] (m22p) at (2,1) {};
\draw[message,colorBlueBase](m22p.center) to (3,0);
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/incremental-average-low-level.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=0.9, every node/.style={scale=0.9},
  thick, colorGrayBase, align=center,
  node distance=1cm and 1.5cm,
  task/.style={rectangle, rounded corners=1mm, very thick, draw,text=black,inner sep=2mm,fill=colorGrayBack},
  taskConnection/.style={-{Triangle[angle=45:5]}, very thick, controls={+(right:1.5) and +(left:1.5)}},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12}
]

\node[scale=0,label={\footnotesize\emph{source}},label={below:integers}] (t0) at (0,0) {};
\draw[taskConnection,{>[angle=45:5]}-]($(t0.west)+(-3.5,0)$) -- (t0.west) node[pos=0.35,above] {\footnotesize \integerEvent{9} \integerEvent{3} \integerEvent{1}};
\node[scale=0,above=of t0,label={\footnotesize\emph{source}},label={below:reset}] (t1) {};
\draw[taskConnection,{>[angle=45:5]}-]($(t1.west)+(-2,0)$) -- (t1.west) node[pos=0.3,above] {\footnotesize \resetEvent};

\node[task,right=of t0,label={\footnotesize\emph{task}}] (t2) {incremental\\average};
\draw[taskConnection](t0.east) to (t2.west);
\draw[taskConnection](t1.east) to ($(t2.west)+(0,0.3)$);

\node[scale=0,right=of t2,label={\footnotesize\emph{sink}},label={below:result}] (t3) {};
\draw[taskConnection,-](t2.east) to (t3.west);
\draw[taskConnection](t3.east) -- ($(t3.east)+(1.5,0)$);
\end{tikzpicture}
\else
hideTikz is set
\fi


==> figures/splitter/explanation.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=\tikzscale, every node/.style={scale=\tikzscale},
  pin distance=3m,
  thick, colorGrayBase,
  node distance=0.3cm*\tikzscale and 1mm*\tikzscale,
  task/.style={rectangle, rounded corners=1mm, very thick, draw,text=black,inner sep=2mm,colorRedBase,fill=colorRedBack},
  event/.style={scale=0.32, rectangle, rounded corners=2mm, text height={2.4mm}, thick, draw, node on layer=foreground,colorGrayBase},
  border/.style={scale=0.275, rectangle, very thick, draw, colorRedEmph, fill=colorRedBack, sloped, rotate=90, node on layer=foreground},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12}
]
\begin{scope}[on background layer]
\draw[double distance=1.5mm*\tikzscale] (0,0) -- (2, 0) node[pos=1/7,event] (e5) {to} node[pos=2/7,event] (e4) {be} node[pos=3/7,event] (e3) {or} node[pos=4/7,event] (e2) {not} node[pos=5/7,event] (e1) {to} node[pos=6/7,event] (e0) {be};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (0,0) -- (2, 0);
\draw[double distance=1.5mm*\tikzscale] (2,0) -- (3, 0) node[pos=1-6/7,event,densely dotted] (e20) {or} node[pos=1-4/7,event,densely dotted] (e10) {be} node[pos=1-2/7,event,densely dotted] (e00) {to};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (2,0) -- (3, 0);
\draw[double distance=1.5mm*\tikzscale,white] (3,0) -- (4, 0);
\node[below=of e5.center,scale=0.25,yshift=8mm] (e5l) {$8$};
\node[below=of e4.center,scale=0.25,yshift=8mm] (e4l) {$7$};
\node[below=of e3.center,scale=0.25,yshift=8mm] (e3l) {$6$};
\node[below=of e2.center,scale=0.25,yshift=8mm] (e2l) {$5$};
\node[below=of e1.center,scale=0.25,yshift=8mm] (e1l) {$4$};
\node[below=of e0.center,scale=0.25,yshift=8mm] (e0l) {$3$};
\node[scale=0.6,inlineImage] at ($(e20.center)+(-0.21,0)$) {\failureImage};
\node[below=of e20.center,scale=0.25,yshift=8mm] (e20l) {$2$};
\node[below=of e10.center,scale=0.25,yshift=8mm] (e10l) {$1$};
\node[below=of e00.center,scale=0.25,yshift=8mm] (e00l) {$0$};
\end{scope}
\begin{scope}[on background layer]
\draw[double distance=1.5mm*\tikzscale] (0,-0.5) -- (2, -0.5) node[pos=1/7,event] (e5n) {to} node[pos=2/7,event] (e4n) {be} node[pos=3/7,event] (e3n) {or} node[pos=4/7,event] (e2n) {not} node[pos=5/7,event] (e1n) {to} node[pos=6/7,event] (e0n) {be};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (0,-0.5) -- (2, -0.5);
\draw[double distance=1.5mm*\tikzscale,white] (2,-0.5) -- (4, -0.5);
\node[below=of e5n.center,scale=0.25,yshift=8mm] {$5$};
\node[below=of e4n.center,scale=0.25,yshift=8mm] {$4$};
\node[below=of e3n.center,scale=0.25,yshift=8mm] {$3$};
\node[below=of e2n.center,scale=0.25,yshift=8mm] {$2$};
\node[below=of e1n.center,scale=0.25,yshift=8mm] {$1$};
\node[below=of e0n.center,scale=0.25,yshift=8mm] {$0$};
\node[right=of e0n.center,scale=0.3,xshift=8mm] {\emph{A failure-free trace}};
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e5l) -- (e5n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e4l) -- (e4n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e3l) -- (e3n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e2l) -- (e2n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e1l) -- (e1n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e0l) -- (e0n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e20l) ..controls +(down:0.1) and +(up:0.35).. (e0n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e10l) ..controls +(down:0.2) and +(up:0.3).. (e0n);
\draw[colorGrayBase,-{Triangle[angle=45:5]}] (e00l) ..controls +(down:0.3) and +(up:0.25).. (e0n);
\end{scope}
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/splitter/failed.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=\tikzscale, every node/.style={scale=\tikzscale},
  pin distance=3m,
  thick, colorGrayBase,
  node distance=0.3cm*\tikzscale and 1mm*\tikzscale,
  task/.style={rectangle, rounded corners=1mm, very thick, draw,text=black,inner sep=2mm,colorRedBase,fill=colorRedBack},
  event/.style={scale=0.32, rectangle, rounded corners=2mm, text height={2.4mm}, thick, draw, node on layer=foreground,colorGrayBase},
  border/.style={scale=0.275, rectangle, very thick, draw, colorRedEmph, fill=colorRedBack, sloped, rotate=90, node on layer=foreground},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12}
]
\begin{scope}[on background layer]
\draw[double distance=1.5mm*\tikzscale] (0,0) -- (2, 0) node[pos=1/7,event] (e5) {to} node[pos=2/7,event] (e4) {be} node[pos=3/7,event] (e3) {or} node[pos=4/7,event] (e2) {not} node[pos=5/7,event] (e1) {to} node[pos=6/7,event] (e0) {be};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (0,0) -- (2, 0);
\draw[double distance=1.5mm*\tikzscale] (2,0) -- (3, 0) node[pos=1-6/7,event,densely dotted] (e20) {or} node[pos=1-4/7,event,densely dotted] (e10) {be} node[pos=1-2/7,event,densely dotted] (e00) {to};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (2,0) -- (3, 0);
\draw[double distance=1.5mm*\tikzscale,white] (3,0) -- (4, 0);
\node[below=of e5.center,scale=0.25,yshift=8mm] {$8$};
\node[below=of e4.center,scale=0.25,yshift=8mm] {$7$};
\node[below=of e3.center,scale=0.25,yshift=8mm] {$6$};
\node[below=of e2.center,scale=0.25,yshift=8mm] {$5$};
\node[below=of e1.center,scale=0.25,yshift=8mm] {$4$};
\node[below=of e0.center,scale=0.25,yshift=8mm] {$3$};
\node[scale=0.6,inlineImage] at ($(e20.center)+(-0.21,0)$) {\failureImage};
\node[below=of e20.center,scale=0.25,yshift=8mm] {$2$};
\node[below=of e10.center,scale=0.25,yshift=8mm] {$1$};
\node[below=of e00.center,scale=0.25,yshift=8mm] {$0$};
\end{scope}
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/splitter/ideal.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=\tikzscale, every node/.style={scale=\tikzscale},
  pin distance=3m,
  thick, colorGrayBase,
  node distance=0.3cm*\tikzscale and 1mm*\tikzscale,
  task/.style={rectangle, rounded corners=1mm, very thick, draw,text=black,inner sep=2mm,colorRedBase,fill=colorRedBack},
  event/.style={scale=0.32, rectangle, rounded corners=2mm, text height={2.4mm}, thick, draw, node on layer=foreground,colorGrayBase},
  border/.style={scale=0.275, rectangle, very thick, draw, colorRedEmph, fill=colorRedBack, sloped, rotate=90, node on layer=foreground},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12}
]
\begin{scope}[on background layer]
\draw[double distance=1.5mm*\tikzscale] (0,0) -- (2, 0) node[pos=1/7,event] (e5) {be} node[pos=2/7,event] (e4) {to} node[pos=3/7,event] (e3) {not} node[pos=4/7,event] (e2) {or} node[pos=5/7,event] (e1) {be} node[pos=6/7,event] (e0) {to};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (0,0) -- (2, 0);
\node[below=of e5.center,scale=0.25,yshift=8mm] {$5$};
\node[below=of e4.center,scale=0.25,yshift=8mm] {$4$};
\node[below=of e3.center,scale=0.25,yshift=8mm] {$3$};
\node[below=of e2.center,scale=0.25,yshift=8mm] {$2$};
\node[below=of e1.center,scale=0.25,yshift=8mm] {$1$};
\node[below=of e0.center,scale=0.25,yshift=8mm] {$0$};
\end{scope}
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/splitter/partial.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=\tikzscale, every node/.style={scale=\tikzscale},
  pin distance=3m,
  thick, colorGrayBase,
  node distance=0.3cm*\tikzscale and 1mm*\tikzscale,
  task/.style={rectangle, rounded corners=1mm, very thick, draw,text=black,inner sep=2mm,colorRedBase,fill=colorRedBack},
  event/.style={scale=0.32, rectangle, rounded corners=2mm, text height={2.4mm}, thick, draw, node on layer=foreground,colorGrayBase},
  border/.style={scale=0.275, rectangle, very thick, draw, colorRedEmph, fill=colorRedBack, sloped, rotate=90, node on layer=foreground},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12}
]
\begin{scope}[on background layer]
\draw[double distance=1.5mm*\tikzscale] (0,0) -- (2, 0) node[pos=4/7,event] (e2) {or} node[pos=5/7,event] (e1) {be} node[pos=6/7,event] (e0) {to};
\draw[line width=1.5mm*\tikzscale,colorGrayBack] (0,0) -- (2, 0);
\node[below=of e2.center,scale=0.25,yshift=8mm] {$2$};
\node[below=of e1.center,scale=0.25,yshift=8mm] {$1$};
\node[below=of e0.center,scale=0.25,yshift=8mm] {$0$};
\end{scope}
\end{tikzpicture}
\else
hideTikz is set
\fi

==> figures/splitter/splitter.tex <==
\ifx\hideTikz\undefined
\begin{tikzpicture}[
  scale=1, every node/.style={scale=1},
  thick, colorGrayBase, align=center,
  node distance=0.5cm and 1cm,
  task/.style={rectangle, rounded corners=1mm, very thick, draw,text=black,inner sep=2mm,fill=colorGrayBack},
  taskConnection/.style={-{Triangle[angle=45:5]}, very thick, controls={+(right:0.5) and +(left:0.5)}},
  inlineImage/.style={scale=0.35, yscale=-1, xshift=-12, yshift=-12}
]

\node[text height=3mm] (input) {``to be or not to be''};

\node[task,base right=of input] (task) {splitter};
\draw[taskConnection,{>[angle=45:5]}-{Triangle[angle=45:5]}](input.east |- task.west)--(task.west);

\node[text height=3mm,base right=of task] (output) {[``to'', ``be'', ``or'', ``not'', ``to'', ``be'']};
\draw[taskConnection](task.east) -- (task.east -| output.west);
\end{tikzpicture}
\else
hideTikz is set
\fi

==> utilities.tex <==
% Custom utility commands
\makeatletter
\newcommand{\labeltext}[2]{%
  \@bsphack
  \csname phantomsection\endcsname
  \def\@currentlabel{#1}{\label{#2}}%
  \@esphack
}
\newcommand{\prflabel}[2]{\label{#2:util}\labeltext{\Cref*{#2} \S~Proof of \Cref*{#1}}{#2}}
\newcommand{\parlabel}[1]{\label{#1:util}\labeltext{\Cref*{#1} \S~\nameref*{#1}}{#1}}

\ifx\showNotesOf\undefined
\newcommand{\todonote}[4]{}
\else
\newcommand{\todonote}[4]{\IfSubStr{\showNotesOf}{#4}{\textup{\colorbox{#2}{\textbf{\color{#3}#4}}~\emph{#1}~{\color{#2}$\blacktriangleleft$}}}{}}
\fi
\newcommand{\av}[1]{\todonote{#1}{yellow}{black}{AV}}
\newcommand{\js}[1]{\todonote{#1}{cyan}{white}{JS}}
\newcommand{\pc}[1]{\todonote{#1}{magenta}{white}{PC}}
\newcommand{\ph}[1]{\todonote{#1}{lime}{black}{PH}}

\newcommand{\suchthat}{\emph{s.t.~}}
\newcommand{\ie}{\emph{i.e.,~}}
\newcommand{\eg}{\emph{e.g.,~}}
\newcommand{\cf}{\emph{cf.~}}

\newcommand{\mathsc}[1]{{\normalfont\textsc{#1}}}

\newcommand{\set}[1]{\bigl\{#1\bigr\}}
\newcommand{\setbuild}[2]{\bigl\{#1\ \big|\ #2\bigr\}}
\newcommand{\map}[2]{\bigl[#1 \mapsto #2\bigr]}
\newcommand{\mapbuild}[3]{\bigl[#1 \mapsto #2\ \big|\ #3\bigr]}
\newcommand{\seq}[3]{\bigl[#1\bigr]_{#2}^{#3}}

\newcommand{\sset}[1]{\left\{#1\right\}}
\newcommand{\ssetbuild}[2]{\left\{#1\ \middle|\ #2\right\}}
\newcommand{\smap}[2]{\left[#1 \mapsto #2\right]}
\newcommand{\smapbuild}[3]{\left[#1 \mapsto #2\ \middle|\ #3\right]}
\newcommand{\sseq}[3]{\left[#1\right]_{#2}^{#3}}

\newcommand{\size}[1]{\left|#1\right|}
\newcommand{\concat}{:}
\newcommand{\single}[1]{\bigl[#1\bigr]}
\newcommand{\ssingle}[1]{\left[#1\right]}
\newcommand{\dom}[1]{\mathrm{dom}(#1)}
\newcommand{\gce}[1]{\mathrm{gce}(#1)}
\newcommand{\lcs}[1]{\mathrm{lcs}(#1)}

\newcommand{\rotor}[5]{#1 ~\,^{#2}\negmedspace\xrightleftharpoons{#3}\!^{#4}\, #5}
\newcommand{\executions}[2]{\mathbb{E}_{#1}^{#2}}
\newcommand{\failuretransparent}[4]{#1 R \bbslash_{#2}^{#3} #4}
\newcommand{\configuration}[5]{\langle\, #1,\, #2,\, #3,\, #4,\, #5 \,\rangle}

\newcommand{\rulesI}{\mathrm{I}}
\newcommand{\rulesF}{\mathrm{F}}

\newenvironment{Figure}{
  \par\noindent\\\begin{minipage}{\textwidth}\raggedright~\captionsetup{type=figure}\\
}{\end{minipage}}
\makeatother

\ifx\disableLinenumbers\undefined\else
\nolinenumbers % temporary remove line numbers
\fi

\newcommand{\techReport}[1]{\ifx\showTechReport\undefined\else#1\fi}
\newcommand{\mainReport}[1]{\ifx\showMainReport\undefined\else#1\fi}
\newcommand{\appRef}[1]{\techReport{\ref{#1}}\mainReport{The complete proof is available in the companion technical report~\cite{veresov2024technicalreport}}}
\newcommand{\appCite}[2]{\techReport{(\Cref{#1})}\mainReport{\cite[#2]{veresov2024technicalreport}}}

%% Jonas' Proof Styles
% Utils
\newcommand{\boxsizesmall}{1cm}
\newcommand{\boxsizelarge}{1.7cm}
\newcommand{\format}[2][\boxsizesmall]{\makebox[#1][l]{\emph{#2}}}
\newcommand{\singleitem}[1]{\begin{enumerate} \item[$\triangleright$] #1 \end{enumerate}}

% Commands
\newcommand{\assume}{\noindent\format[\boxsizelarge]{Assume:~}}
\newcommand{\prove}{\noindent\format[\boxsizelarge]{Prove:~}}
\newcommand{\where}{\noindent\format{Where:~}}
\newcommand{\suffices}{\noindent\format[\boxsizelarge]{Suffices:~}}
\newcommand{\expand}{\noindent\format[\boxsizelarge]{Expanded:~}}
\newcommand{\new}{\format{New:~}}
\newcommand{\letdef}{\format{Let:~}}
\newcommand{\pick}{\format{Pick:~}}
\newcommand{\case}{\format{Case:~}}
\newcommand{\proofby}[1]{\singleitem{\format{Proof:~} #1}}
\newcommand{\proofbyitem}[1]{\item[]\hspace{\parindent}$\triangleright$\hspace{\labelsep}\format{Proof:~} #1}% to be used when there are spacing issues due to consecutive lists
\newcommand{\smallnote}[1]{\singleitem{\format{Note:~} #1}}
\newcommand{\qeditem}{\item \format{QED}}
\newcommand{\highlight}[1]{\colorbox{lipicsLightGray}{\ensuremath{#1}}}

% Hide or show proof notes
\ifx\hideProofNotes\undefined
\newcommand{\handwave}[1]{\textcolor{red}{\format[2cm]{Handwave:~}#1}}
\else
\newcommand{\handwave}[1]{#1}
\fi

